CMT in TREC-COVID Round 2: Mitigating the Generalization Gaps from Web to Special Domain Search

Neural rankers based on deep pretrained language models (LMs) have been shown to improve many information retrieval benchmarks. However, these methods are affected by their the correlation between pretraining domain and target domain and rely on massive fine-tuning relevance labels. Directly applying pretraining methods to specific domains may result in suboptimal search quality because specific domains may have domain adaption problems, such as the COVID domain. This paper presents a search system to alleviate the special domain adaption problem. The system utilizes the domain-adaptive pretraining and few-shot learning technologies to help neural rankers mitigate the domain discrepancy and label scarcity problems. Besides, we also integrate dense retrieval to alleviate traditional sparse retrieval's vocabulary mismatch obstacle. Our system performs the best among the non-manual runs in Round 2 of the TREC-COVID task, which aims to retrieve useful information from scientific literature related to COVID-19. Our code is publicly available at https://github.com/thunlp/OpenMatch.

==> Archive/3_Methodology.tex <==
\section{System Description}\label{sec:system}

This section will showcase our CMT system and describe how each part of the system responds to the above generalization gap.
\zh{First dense retrieval for document retrieval. Then few-shot learning for neural reranking. Finally say our domain specific MLM.}


\subsection{Continuous MLM Training}
~\zh{The fist paragraph can be more general and pay more attention to the differences of general MLM and COVID-targeted MLM. We choose the scibert, tell the differences of bert and scibert. In addition, wht you choose the mask rate 15\%, refer the original bert paper. }
The pre-training masked language model on a domain-specific corpus has been proved to enhance downstream tasks, such as the scientific domain~\cite{Beltagy2019SciBERT}. Followed the direction, we continue to perform MLM training on SciBERT on the CORD19 corpus to ease the cross-domain gap of COVID. CMT system inherits the same architecture and vocabulary as SciBERT and uses WordPiece for unsupervised tokenization of COVID-19 papers. In all of our experiments, we use the full text of the documents, not just the abstracts, and mask 15\% of all WordPiece tokens in each sequence at random.

\subsection{Few-Shot Learning}
~\zh{Say the challenge of COVID-IR and why it is a few-shot task.}
Few-shot learning has been extensively studied to improve model training in the low-data regime~\cite{wang2019few}. Two few-shot learning methods are applied in our system to alleviate COVID's label scarcity, including weak supervision data selection and in-domain data generation.~\zh{Mention the two methods in out models.}

~\zh{The first part should describe the contrastive qg. Tell why we need more COVID-targeted data.}
\textbf{Selective Weak Supervision.} It is natural to regard the rich medical-related annotation in MS-MARCO as weak supervision data for training the neural ranker in the low-resource COVID search. Here we leverage ReInfoSelect~\cite{zhang2020selective}, an advanced data selection method based on reinforcement learning, to distinguish valuable weak supervision signals for robust training.

Given the medical MS-MARCO as the training set, and a few annotated data (TREC-COVID Round 1) as target set, ReInfoSelect uses the policy gradient to propagate the reward signals from target data to a weak supervision data selector, where the evaluation result of the ranker on the target data is used as reward signals. SciBERT is our ranker with warm-up training on the previous MLM stage. 


~\zh{The second part should describe weak supervision selection.}

\textbf{Contrastive Query Generation.} There are also apparent differences between medical MS MARCO and COVID, even that they both belong to the medical field. To further mitigate the gap, we used advances in query generation to construct related query-document pairs in the COVID domain automatically. 

In the first attempt, we trained a generator on the medical MS MARCO, which can generate queries by encoding a single document~\cite{ma2020zero}. But the query generated by the generator trained on query-document pairs is too general, so that the query may be related to many other papers. We propose a simple but effective generation method for generating more distinguishable queries. Instead of encoding a single document to generate related queries, our generator learns to produce queries based on a pair of contrast documents related to but cover different topics. 

The process of obtaining contrast document pair is divided into two steps. First, we considered queries generated in the first attempt as the first generation and then use BM25 to extract relevant documents according to the queries. Then two documents randomly selected from the relevance list returned by BM25 are concatenated and fed to the contrast query generator to generate the second generation query, where the contrast generator was pre-trained on the medical MARCO triples $<$query, positive doc, negative doc$>$.

%% **********************************************************
\input{Diagrams/overall}
\input{Diagrams/rankdepth}
%% **********************************************************
~\zh{This part can be more simplification.}
\subsection{Dense Retrieval}
Dense retrieval standing on distributed representations can compare queries and documents at the semantic level even if they use different vocabularies, which complement to the sparse retriever by design~\cite{gao2020complementing, karpukhin2020dense}. Given this, the CMT system combines sparse BM25 and the dense Approximate Nearest Neighbor (ANN) method.

ANN aims to search the nearest neighbors of documents regarding the similarity between the query $q$ and the document $d$. The core part of ANN is the dense encoder $E(\cdot)$, which is used to maps text to distributed vectors and build an index for all the documents we will use for retrieval. At search-time, the encoder $E(\cdot)$ maps the query to the same distributed representation space and retrieves $k$ documents of which vectors are the closest to the query vector. In our system, we define the similarity between queries and documents as their vectors' dot product and regards BERT as the dense encoder $E(\cdot)$:
$$
sim(q, d) = E(q)^{T}E(d),
$$
Training ANN can formulate as a learning-to-rank problem. Given training dataset $D = \{(q_i, d_{i}^{+}, D_{i}^{-})\}_{i=1}^{N}$ that consists of $N$ instances. Each instance contains a query $q_i$ and its relevant (positive) document $d_{i}^{+}$ along with $m$ irrelevant (negative) documents $D_{i}^{-} = \{d_{ij}^{-}\}_{j=1}^{m}$. The training objective is to learn a distributed space such that the positive document has a higher similarity to the query than all negative documents:
$$
L(q, d^{+}, D^{-}) = \frac{1}{N}\sum_{i=1}^{N}-\text{log}\frac{e^{sim(q_i, d^{+})}}{e^{sim(q_i, d^{+})} + \sum_{j=1}^{m}e^{sim(q_i, d_{ij}^{-})}},
$$
where the training instance comes from medical MS MARCO.







==> Diagrams/bm25_recall.tex <==
\begin{table}[h]
    \centering
    \caption{\label{tab:bm25_recall}The recall rate of BM25 in Round2 of TREC-COVID.}
    \begin{tabular}{c c} \hline 
    R@100 & R@1000 \\
    \hline 
    0.2785 & 0.6573 \\
    \hline
    \end{tabular}
\end{table}

==> Diagrams/oov.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{\label{tab:oov}The OOV rate denotes the proportion of query words out of the vocabulary from TREC-COVID and Medical MS MARCO. The subword rate exhibits the ratio of words divided into sub-words in the WordPiece vocabulary like BERT, etc.}

    \begin{tabular}{l|c c} 
    \hline
    \multirow{2}{*}{\textbf{Vocabulary}} & \multicolumn{2}{c}{\textbf{Query}} \\
    & \textbf{TREC-COVID} & \textbf{MS MARCO} \\ 
    \hline
    \multicolumn{3}{l}{\textbf{OOV Rate}} \\
    \hline
    \text{Glove} & 0.4190 & 0.3402 \\
    \text{BioWordVec} & 0.3905 & 0.3240 \\
    \hline
    \multicolumn{3}{l}{\textbf{Subword Rate}} \\
    \hline
    \text{BioBERT} & 0.5272 & 0.1776 \\
    \text{BERT} & 0.5105 & 0.1366 \\
    \text{SciBERT} & 0.4424 & 0.1201 \\
    \hline
    \end{tabular}
\end{table}

% \begin{table}[t]
%     \centering
%     \small
%     \caption{\label{tab:oov}The Out Of the Vocabulary (OOV) proportion of query words from TREC-COVID and Medical MSMARCO, where words divided into sub-words are considered OOV in the WordPiece vocabulary like BERT, etc.}
%     % \resizebox{0.5\textwidth}{!}{
%     \begin{tabular}{l|c c} 
%     \hline
%     \multirow{2}{*}{\textbf{Vocabulary}} & \multicolumn{2}{c}{\textbf{Query OOV}} \\
%     & \textbf{TREC-COVID} & \textbf{MS MARCO} \\
%     \hline
%     \texttt{Glove} & 0.4190 & 0.3402 \\
%     \texttt{BioWordVec} & 0.3905 & 0.3240 \\
%     \hline
%     \texttt{BioBERT} & 0.5272 & 0.1776 \\
%     \texttt{BERT} & 0.5105 & 0.1366 \\
%     \texttt{SciBERT} & 0.4424 & 0.1201 \\
%     \hline
%     \end{tabular}
%     % }
% \end{table}

==> Diagrams/query_case.tex <==
\begin{table}[h]
    \centering
    \small
    \caption{\label{tab:oov}New Query Cases}
    \begin{tabular}{l|l} 
    \hline \hline
    \multirow{5}{*}{\textbf{R2 New Query}} & \textbf{coronavirus} subtypes \\
    & \textbf{coronavirus} recovery \\
    & \textbf{coronavirus} public datasets \\
    & \textbf{coronavirus} vaccine candidates \\
    & difference between \textbf{coronavirus} and flu \\
    \hline
    \multirow{5}{*}{\textbf{R3 New Query}} & coronavirus mutations \\
    & COVID-19 cytokine storm \\
    & SARS-CoV-2 spike structure \\
    & COVID inflammatory response \\
    & SARS-CoV-2 phylogenetic analysis \\
    \hline \hline
    \end{tabular}
\end{table}


==> Diagrams/years.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.25\textwidth]{Figures/year_distribution.pdf}
\caption{\label{fig:years}Year Distribution of CORD-19 Papers.
}
\end{figure}


==> authorship.tex <==

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
\author{Ben Trovato}
\authornote{Both authors contributed equally to this research.}
\email{trovato@corporation.com}
\orcid{1234-5678-9012}
\author{G.K.M. Tobin}
\authornotemark[1]
\email{webmaster@marysville-ohio.com}
\affiliation{%
  \institution{Institute for Clarity in Documentation}
  \streetaddress{P.O. Box 1212}
  \city{Dublin}
  \state{Ohio}
  \postcode{43017-6221}
}

\author{Lars Th{\o}rv{\"a}ld}
\affiliation{%
  \institution{The Th{\o}rv{\"a}ld Group}
  \streetaddress{1 Th{\o}rv{\"a}ld Circle}
  \city{Hekla}
  \country{Iceland}}
\email{larst@affiliation.org}

\author{Valerie B\'eranger}
\affiliation{%
  \institution{Inria Paris-Rocquencourt}
  \city{Rocquencourt}
  \country{France}
}

\author{Aparna Patel}
\affiliation{%
 \institution{Rajiv Gandhi University}
 \streetaddress{Rono-Hills}
 \city{Doimukh}
 \state{Arunachal Pradesh}
 \country{India}}

\author{Huifen Chan}
\affiliation{%
  \institution{Tsinghua University}
  \streetaddress{30 Shuangqing Rd}
  \city{Haidian Qu}
  \state{Beijing Shi}
  \country{China}}

\author{Charles Palmer}
\affiliation{%
  \institution{Palmer Research Laboratories}
  \streetaddress{8600 Datapoint Drive}
  \city{San Antonio}
  \state{Texas}
  \postcode{78229}}
\email{cpalmer@prl.com}

\author{John Smith}
\affiliation{\institution{The Th{\o}rv{\"a}ld Group}}
\email{jsmith@affiliation.org}

\author{Julius P. Kumquat}
\affiliation{\institution{The Kumquat Consortium}}
\email{jpkumquat@consortium.net}

%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
\renewcommand{\shortauthors}{Trovato and Tobin, et al.}

